Sense Amplifier Comparator with Offset Correction for Decision Feedback Equalization based Receivers

A decision feedback circuit with integrated offset compensation is presented in this paper. The circuit is built around the sense amplifier comparator. The feedback loop is closed around the first stage of the comparator resulting in minimum loop latency. The feedback loop is implemented using a switched capacitor network that picks from one of pre-computed voltages to be fed back. The comparator's offset that is to be compensated for, is added in the same path. Hence, an extra offset correction input is not required. The circuit is used as a receiver for a 10 mm low swing interconnect implemented in UMC 130 nm CMOS technology. The circuit is tested at a frequency of 1 GHz and it consumes 145 $\mu$A from a 1.2V supply at this frequency.

==> abstract.tex <==
\begin{abstract}
A decision feedback circuit with integrated offset compensation 
is presented in this paper. The circuit is built around the sense amplifier 
comparator. The feedback loop is closed around the first stage of the 
comparator resulting in minimum loop latency. The feedback loop is 
implemented using a switched capacitor network that picks from one of 
pre-computed voltages to be fed back. The comparator's offset that is 
to be compensated for, is added  in the same path. Hence, an extra offset 
correction input is not required. The circuit 
is used as a receiver for a 10~mm low swing interconnect implemented in 
UMC 130 nm CMOS technology. The circuit is tested at a frequency of 1~GHz 
and it consumes 145~$\mu$A from a 1.2V supply at this frequency.
%
%Equalization (DFE) and integrated offset compensation 
%is presented. 
%The circuit can be used in clocked receivers 
%for repeaterless interconnects. An example implementation
%of a capacitive transmitter with a 10 mm interconnect 
%in TSMC 65 nm CMOS process for a data rate of 5 Gbps 
%is shown. Layout extracted 
%simulations show that the link consumes () fJ/bit 
%from a 1V supply.
\end{abstract}

